Optimal design of large-scale nonlinear Bayesian inverse problems under model uncertainty

We consider optimal experimental design (OED) for Bayesian nonlinear inverse problems governed by partial differential equations (PDEs) under model uncertainty. Specifically, we consider inverse problems in which, in addition to the inversion parameters, the governing PDEs include secondary uncertain parameters. We focus on problems with infinite-dimensional inversion and secondary parameters and present a scalable computational framework for optimal design of such problems. The proposed approach enables Bayesian inversion and OED under uncertainty within a unified framework. We build on the Bayesian approximation error (BAE) approach, to incorporate modeling uncertainties in the Bayesian inverse problem, and methods for A-optimal design of infinite-dimensional Bayesian nonlinear inverse problems. Specifically, a Gaussian approximation to the posterior at the maximum a posteriori probability point is used to define an uncertainty aware OED objective that is tractable to evaluate and optimize. In particular, the OED objective can be computed at a cost, in the number of PDE solves, that does not grow with the dimension of the discretized inversion and secondary parameters. The OED problem is formulated as a binary bilevel PDE constrained optimization problem and a greedy algorithm, which provides a pragmatic approach, is used to find optimal designs. We demonstrate the effectiveness of the proposed approach for a model inverse problem governed by an elliptic PDE on a three-dimensional domain. Our computational results also highlight the pitfalls of ignoring modeling uncertainties in the OED and/or inference stages.

==> def.tex <==
\makeatletter
\DeclareFontFamily{OMX}{MnSymbolE}{}
\DeclareSymbolFont{MnLargeSymbols}{OMX}{MnSymbolE}{m}{n}
\SetSymbolFont{MnLargeSymbols}{bold}{OMX}{MnSymbolE}{b}{n}
\DeclareFontShape{OMX}{MnSymbolE}{m}{n}{
    <-6>  MnSymbolE5
   <6-7>  MnSymbolE6
   <7-8>  MnSymbolE7
   <8-9>  MnSymbolE8
   <9-10> MnSymbolE9
  <10-12> MnSymbolE10
  <12->   MnSymbolE12
}{}
\DeclareFontShape{OMX}{MnSymbolE}{b}{n}{
    <-6>  MnSymbolE-Bold5
   <6-7>  MnSymbolE-Bold6
   <7-8>  MnSymbolE-Bold7
   <8-9>  MnSymbolE-Bold8
   <9-10> MnSymbolE-Bold9
  <10-12> MnSymbolE-Bold10
  <12->   MnSymbolE-Bold12
}{}

\let\llangle\@undefined
\let\rrangle\@undefined
\DeclareMathDelimiter{\llangle}{\mathopen}%
                     {MnLargeSymbols}{'164}{MnLargeSymbols}{'164}
\DeclareMathDelimiter{\rrangle}{\mathclose}%
                     {MnLargeSymbols}{'171}{MnLargeSymbols}{'171}
\makeatother



% -------------------------------------------------------------------
% packages 
% -------------------------------------------------------------------

\expandafter\let\csname equation*\endcsname\relax
\expandafter\let\csname endequation*\endcsname\relax
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}


\usepackage[margin=1in]{geometry}
\usepackage{booktabs}
\usepackage{mathrsfs}
\usepackage{euscript}
\usepackage[scr=rsfso]{mathalfa}
\usepackage{color}
\usepackage{graphicx}
\usepackage{algorithmic,algorithm} 
\usepackage{tikz,pgfplots}
\usepackage{upgreek}
\usepackage{showkeys,cite}
\usepackage{multirow}
\usepackage{yfonts}
\usepackage{mathtools}
\usepackage[normalem]{ulem}
\usepackage{latexsym}
\usepackage{url} 
\usepackage{braket,amsfonts}
\usepackage{float}
\usepackage{tabu}
\usepackage{epstopdf}
\usepackage{enumitem}
\usepackage{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor=blue,
    citecolor=blue,
    filecolor=blue,      
    urlcolor=blue,
    }
\usepackage{cleveref}

\usepackage{etoolbox}

\newcommand{\cfootnote}[2][black]{%
    {\color{#1}\footnote{#2}}%
}


%\usepackage[hang]{footmisc}


\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}
\DeclareMathAlphabet      {\mathup}{OT1}{\familydefault}{m}{n}


% -------------------------------------------------------------------
% definitions
% -------------------------------------------------------------------
% colors, etc
\definecolor{grassgreen}{RGB}{92,135,39}

% -------------------------------------------------------------------
% macros
% -------------------------------------------------------------------

% general 


\newcommand{\hilb}{\mathscr{H}}
\newcommand{\hilbm}{\mathscr{M}}
\newcommand{\hilbb}{\mathscr{X}}
\newcommand{\hilbn}{\mathscr{V}_n}
\newcommand{\defeq}{\vcentcolon=}
\renewcommand{\vec}[1]{{\mathchoice
                     {\mbox{\boldmath$\displaystyle{#1}$}}
                     {\mbox{\boldmath$\textstyle{#1}$}}
                     {\mbox{\boldmath$\scriptstyle{#1}$}}
                     {\mbox{\boldmath$\scriptscriptstyle{#1}$}}}}
\renewcommand{\mat}[1]{\mathbf{{#1}}}
\renewcommand{\ker}{\mathsf{ker}}
\newcommand{\ran}{\mathsf{range}}
\newcommand{\dom}{\mathsf{dom}}
\newcommand{\trace}{\mathsf{tr}}
\newcommand{\eps}{\varepsilon}
\newcommand{\norm}[1]{\left\| {#1} \right\|}


% the various inner products:
\newcommand{\ip}[2]{{\langle {#1},{#2} \rangle}}            % generic
\newcommand{\ipp}[3]{{\langle {#2}, {#3} \rangle}_{{#1}}}   % general purpose command
\newcommand{\mip}[2]{\ipp{\!\hilbm}{#1}{#2}}                  % inner product on inversion param space
\newcommand{\cip}[2]{\ipp{\CM}{#1}{#2}}                     % Cameron--Martin inner product
\newcommand{\eip}[2]{\ipp{\R^q}{#1}{#2}}                    % Euclidean inner product


\newcommand{\grad}{\nabla}
\newcommand\restr[2]{{
  \left.\kern-\nulldelimiterspace % automatically resize the bar with \right
  {#1}\vphantom{\big|} \right|_{#2}}}

% sets of numbers 
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}

\newcommand{\QoI}{\Theta}
\newcommand\gauss[2]{1/(#2*sqrt(2*pi))*exp(-((x-#1)^2)/(2*#2^2))} % Gauss function, parameters mu and sigma
\newcommand{\ctrl}{\vec{z}}
\newcommand{\Nc}{{n_\text{c}}}

\usetikzlibrary{calc}
\tikzset{
    state/.style={
           rectangle,
           rounded corners,
           draw=black, very thick,
           minimum height=3em,
           inner sep=1pt,
           text centered,
           },
}



%
% commonly used mathcals, etc
%
\newcommand{\A}{\mathcal{A}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\K}{\mathcal{K}}
\renewcommand{\S}{\mathcal{S}}
\newcommand{\RR}{\mathcal{R}}
\newcommand{\J}{\mathcal{J}}
\newcommand{\U}{\mathcal{U}}
\newcommand{\JL}{\mathcal{J}_{\!L}}

\newcommand{\E}{\mathcal{E}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\G}{\mathcal{G}}

\newcommand{\FF}{\mat{F}}
\newcommand{\II}{\mat{I}}
\newcommand{\GG}{\mat{G}}

% Probability (general)
\newcommand{\prob}{\mathsf{Prob}}
\newcommand{\borel}{\mathfrak{B}}
\newcommand{\var}{\mathsf{Var}}
\newcommand{\ave}{\mathsf{E}}
\newcommand{\GM}[2]{\mathcal{N}\!\left( {#1}, {#2}\right)}


% Bayesian stuff

\newcommand{\Cprior}{\mathcal{C}_{\mathup{pr}}}
\newcommand{\Cpost}{\mathcal{C}_{\mathup{post}}}
\newcommand{\ncov}{\mat{\Gamma}_{\mathup{noise}}}
\newcommand{\ecov}{\mat{\Gamma}_{\mathup{\eps}}}
\newcommand{\ecovhat}{\widehat{\mat{\Gamma}}_{\mathup{\eps}}}
\newcommand{\nucov}{\mat{\Gamma}_{\mathup{\nu}}}
\newcommand{\nucovw}{\mat{\Gamma}_{\mathup{\nu},\vec{w}}}
\newcommand{\mcov}{\mat{\Gamma}_{\mathup{model}}}
\newcommand{\noisem}{\mu_{\mathup{noise}}}
\newcommand{\like}{\Pi_{\mathup{like}}^{\scriptscriptstyle\mathup{BAE}}}
\newcommand{\noise}{\Pi_\text{noise}}
\newcommand{\obs}{\vec{y}}
\newcommand{\ipar}{\theta}
\newcommand{\iparm}{m}
\newcommand{\iparb}{\xi}
\newcommand{\iparpost}{\ipar_{\mathup{post}}}
\newcommand{\iparpostm}{\iparm_{\mathup{post}}}
\newcommand{\iparpostb}{\iparb_{\mathup{post}}}
\newcommand{\iparpr}{\ipar_{\mathup{pr}}}
\newcommand{\iparprm}{m_{\mathup{pr}}}
\newcommand{\iparprb}{b_{\mathup{pr}}}
\newcommand{\iparmap}{m_{\scriptscriptstyle\mathup{MAP}}}
\newcommand{\dpar}{\vec{\theta}}
\newcommand{\dparm}{\vec{m}}
\newcommand{\dparb}{\vec{b}}
\newcommand{\dparpr}{\dpar_{\mathup{pr}}}
\newcommand{\dparprm}{\dparm_{\mathup{pr}}}
\newcommand{\dparprb}{\dparb_{\mathup{pr}}}
\newcommand{\dparmap}{\dpar_{\scriptscriptstyle\mathup{MAP}}}
\newcommand{\dparmapm}{\vec{m}_{\scriptscriptstyle\mathup{MAP}}}
\newcommand{\dparmapb}{\vec{b}_{\scriptscriptstyle\mathup{MAP}}}
\newcommand{\iprcov}{\Gamma_{\mathup{pr}}}
\newcommand{\iprcovm}{\Gamma_{\mathup{pr,m}}}
\newcommand{\iprcovb}{\Gamma_{\mathup{pr,b}}}
\newcommand{\ipostcov}{\Gamma_{\mathup{post}}}
\newcommand{\prcovm}{\mat{\Gamma}_{\mathup{pr,m}} }
\newcommand{\prcovb}{\mat{\Gamma}_{\mathup{pr,b}} }
\newcommand{\prcov}{\mat{\Gamma}_{\mathup{pr}} }
\newcommand{\postcov}{\mat{\Gamma}_{\mathup{post}} }
\newcommand{\postcovm}{\mat{\Gamma}_{\mathup{post},\mathup{m}} }
\newcommand{\postcovmb}{\mat{\Gamma}_{\mathup{post},\mathup{mb}} }
\newcommand{\postcovb}{\mat{\Gamma}_{\mathup{post},\mathup{b}} }
\newcommand{\prior}{\mu_{\mathup{pr}}}
\newcommand{\priorm}{\mu_{\mathup{pr,m}}}
\newcommand{\priorb}{\mu_{\mathup{pr,b}}}
\newcommand{\postmSimp}{\mu_{\mathup{post}}}
\newcommand{\postmGSimp}{{\hat\mu}_{\mathup{post}}}
\newcommand{\postm}{\mu_{\mathup{post}}^\obs}
\newcommand{\postmG}{{\hat\mu}_{\mathup{post}}^\obs}
\newcommand{\postmGw}{{\hat\mu}_{\mathup{post}}^{\obs, \vec w}}
\newcommand{\postmw}{\mu_{\mathup{post}}^{\obs,\vec{w}}}
\newcommand{\M}{\mat{M}}                       % the Mass matrix
\newcommand{\ff}{\vec{f}}                      % parameter-to-obs MAP
\newcommand{\Nw}{{n_w}}
\newcommand{\mOED}{{mOED}}
\newcommand{\mOEDs}{{mOEDs}}


% custom commands (add your own macros here) 
\newcommand{\Nm}{{n_\text{m}}}
\newcommand{\Nb}{{n_\text{b}}}
\newcommand{\Ns}{{n_\text{s}}}
\newcommand{\Nd}{{n_\text{d}}}
\newcommand{\Nv}{{n_\text{v}}}
\newcommand{\Nsamp}{{n_\text{mc}}}
\newcommand{\Ntr}{{n_{\text{tr}}}}
\newcommand{\Nact}{{n_{\text{act}}}}
\newcommand{\axsp}{{\mathcal{M}}}
\newcommand{\jtsp}{{\mathcal{V}}}
\newcommand{\afwd}{\mathcal{G}}
\newcommand{\cfwd}{\mathcal{F}}
\newcommand{\flin}{\mathcal{L}}



\renewcommand{\H}{\mathcal{H}}
\newcommand{\HT}{\widetilde{\mathcal{H}}}
\newcommand{\obj}{\Psi}
\newcommand{\objG}{\obj^{\scriptscriptstyle{\mathup{G}}}}
\newcommand{\eeta}{\vec{\eta}}
\newcommand{\CM}{\mathscr{E}}
\newcommand{\W}{\mat{W}}
\newcommand{\Wn}{\mat{W}_{\!\!\upsigma}}
\newcommand{\yhati}{{\obs^{i}_{\!\vec w}}}
\newcommand{\mi}{\iparm_i^\star}
\newcommand{\yhatip}{{\mathbf{d}^{i}_{\vec w}}}
\newcommand{\yhat}{{\obs_{\!\vec w}}}
\newcommand{\PPsi}{\mat{P}_{\!\vec{w}}}
\newcommand{\WW}{\mat{\Sigma}}

\newcommand{\sn}{\sigma^2_{\mathup{noise}}}
\newcommand{\HM}{\H_{\mathup{misfit}}}
\newcommand{\HMt}{\tilde\H_{\mathup{misfit}}}
\newcommand{\HMd}{\mat{H}_{\mathup{misfit}}}
\newcommand{\ad}[1]{{#1}^\ast}
\newcommand{\adfd}[1]{\vec{{#1}}^\ast}
\newcommand{\ut}[1]{\ensuremath{\tilde{#1}}}
\newcommand{\Reg}{\Cprior^{-1}}
\newcommand{\Exp}[1]{e^{{#1}}}
\newcommand{\ipart}{m_{\scriptscriptstyle\mathup{true}}}
\newcommand{\commentout}[1]{\iffalse {#1} \fi}
\newcommand{\alennote}[1]{\noindent\emph{\textcolor{blue}{Alen: #1\,}}}
\newcommand{\nnote}[1]{\noindent\emph{\textcolor{grassgreen}{N: #1\,}}}
\newcommand{\gsnote}[1]{\noindent\emph{\textcolor{orange}{GS: #1\,}}}
\newcommand{\runote}[1]{\noindent\emph{\textcolor{violet}{Ru: #1\,}}}
\newcommand{\V}{\mathscr{V}_{\!\scriptscriptstyle{0}}}
\newcommand{\Vg}{\mathscr{V}_{\!g}}
%\newcommand{\V}{\mathscr{V}}
%\newcommand{\Vg}{\mathscr{U}}
\newcommand{\tran}{{\mkern-1.5mu\mathsf{T}}}                % Transpose
\newcommand{\adj}{{\mkern-1.5mu{*}}}                % Transpose

\newcommand{\FG}{\mat{C}}
\newcommand{\FPF}{\mat{D}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\MM}{\mathbb{M}}
\newcommand{\EE}{\mat{E}}
\newcommand{\rr}{\vec{r}}
\newcommand{\mm}{\vec{m}}
\newcommand{\iparr}{r}

\newcommand{\Snm}{S^{\mat{M}}_{++}}
\newcommand{\DT}{\mathcal{T}}
\newcommand{\Q}{{\mat{Q}}}
\newcommand{\isaacnote}[1]{{\color{purple}Isaac : {#1}}}

\newcommand{\GN}{\ensuremath{\Gamma_{\!\text{N}}}}
\newcommand{\GR}{\ensuremath{\Gamma_{\!\text{R}}}}
\newcommand{\GD}{\ensuremath{\Gamma_{\!\text{D}}}}

\newcommand{\Gq}{\Gamma_{\!\mathup{q}}(\vec{w})}

\newcommand{\LI}{\mathscr{L}^{{{\text{I}}}}}
\newcommand{\tab}{\,\,\,\,}
\DeclareMathOperator*{\argmin}{arg\,min}

\renewcommand{\SS}{\mathcal{S}}
\newcommand{\TT}{\mathcal{T}}
\newcommand{\Caux}{\mathcal{C}_{\iparb}}

\newcommand{\utest}{\ensuremath{\tilde{p}}}
\newcommand{\ptest}{\ensuremath{\tilde{u}}}
\newcommand{\ytest}{\ensuremath{\tilde{y}}}
\newcommand{\mtest}{\ensuremath{\tilde{m}}}

\newcommand{\mhat}{\ensuremath{\hat{m}}}

\newcommand{\PhiNdTR}{\Phi_{\Nd}^{\mathrm{tr}}}
\newcommand{\PhiNdLR}{\Phi_{\Nd}^{\mathrm{eig}}}
\newcommand{\PhiNdLRr}{\Phi_{\Nd,r}^{\mathrm{eig}}}
\newcommand{\PhiNdLRinf}{\Phi_{\Nd,\Ns}^{\mathrm{eig}}}

\newcommand{\centered}[1]{\begin{tabular}{l} #1 \end{tabular}}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}



\crefname{subsection}{section}{sections}
\Crefname{subsection}{Section}{sections}
\crefname{equation}{}{}



% extra ...
%\newcommand{\qip}[2]{\left\langle{#1}, {#2}\right\rangle_{\!\scriptscriptstyle{\mathbb{Q}}}}
%\newcommand{\mip}[2]{\left\langle{#1}, {#2}\right\rangle_{\!\scriptscriptstyle{\mathbb{M}}}}

% spaces of linear transformations
\def\Plus{\texttt{+}}
\renewcommand{\L}{\mathscr{L}}
\newcommand{\Lsym}{\L^\text{sym}}
\newcommand{\Lsymp}{\L^\text{sym\Plus}}
\newcommand{\Lt}{\L_1}
\newcommand{\Ltsym}{\L_1^\text{sym}}
\newcommand{\Ltsymp}{\L_1^\text{sym\Plus}}
\newcommand{\Ltsympp}{\L_1^\text{sym\Plus\Plus}}

\newcommand{\diag}{\mathop{\mathrm{diag}}}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}{Corollary}[theorem]

% for convenience
\newcommand{\vrl}{\obs - \flin(\iparm) - \vec{\eps}_0}
\newcommand{\vrf}{\obs - \cfwd(\iparm) - \vec{\eps}_0}
\newcommand{\vrfmap}{\obs - \cfwd(\iparmap) - \vec{\eps}_0}
